Asking Clarification Questions to Handle Ambiguity in Open-Domain QA

Ambiguous questions persist in open-domain question answering, because formulating a precise question with a unique answer is often challenging. Previously, Min et al. (2020) have tackled this issue by generating disambiguated questions for all possible interpretations of the ambiguous question. This can be effective, but not ideal for providing an answer to the user. Instead, we propose to ask a clarification question, where the user's response will help identify the interpretation that best aligns with the user's intention. We first present CAMBIGNQ, a dataset consisting of 5,654 ambiguous questions, each with relevant passages, possible answers, and a clarification question. The clarification questions were efficiently created by generating them using InstructGPT and manually revising them as necessary. We then define a pipeline of tasks and design appropriate evaluation metrics. Lastly, we achieve 61.3 F1 on ambiguity detection and 40.5 F1 on clarification-based QA, providing strong baselines for future work.

==> TABLES/cq_examples.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll}
\toprule
Ambiguous Question& {Who is the current chairman of african union commission?} \\\cline{1-2}

Reference CQ & {\texttt{\textcolor{orange}{Which chairman}}: \textcolor{blue}{4th}, \textcolor{blue}{3rd}, or \textcolor{blue}{2nd}?} \\
Predicted CQ from BART & {\texttt{\textcolor{orange}{Which year}}: \textcolor{blue}{2017}, or \textcolor{blue}{2012}?}  \\\cline{1-2}

AQ revised by \texttt{$\hat{opt_1}$ - \textcolor{blue}{2017}} & {Who is the current chairman of african union commission, \texttt{\textcolor{orange}{which year}}: \textcolor{blue}{\texttt{2017}}?} \\
AQ revised by \texttt{$\hat{opt_2}$ - \textcolor{blue}{2012}} & {Who is the current chairman of african union commission, \texttt{\textcolor{orange}{which year}}: \textcolor{blue}{\texttt{2012}}?} \\ 
\bottomrule
\end{tabular}%
}
\caption{
Examples of clarification questions (CQs) and ambiguous questions (AQ) revised by the generated CQ.
\todo{Is this table necessary? If not, remove it and you can refer to Table 3.}
}
\label{tab:cq_examples}
\vspace{-5mm}
\end{table*}
% option, ap 만 잡아도 됨. AP만 색깔로 하는걸 본문에 넣고 appendix 에 투컬럼으로 





% % & Ans: \texttt{November 7, 2014 | October   2, 2015 | 18 November 2016}\\      
% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{ll}
% \toprule
% Ambiguous Question& \texttt{When did the samsung gear s come out?} \\
% Reference CQ from auto-conversion & \texttt{Could you clarify 'the samsung gear s'--'original', 'samsung gear s2', or 'samsung gear s3'?} \\
% Generated CQ from BART & \texttt{Could you clarify 'the samsung gear s'--'first' or '2nd'?}  \\
% (`the samsung gear s', `first')-DQ& \texttt{When did the samsung gear s \textbf{first} come out?} \\
% (`the samsung gear s', `second')-DQ& \texttt{When did the samsung gear s \textbf{second} come out?} \\ 
% \bottomrule
% \end{tabular}%
% }
% \caption{
% Examples of clarification questions (CQs) and disambiguated questions (DQs) by the generated CQ.
% }
% \label{tab:cq_examples}
% \end{table*}
% % option, ap 만 잡아도 됨. AP만 색깔로 하는걸 본문에 넣고 appendix 에 투컬럼으로 


% % & Ans: \texttt{November 7, 2014 | October   2, 2015 | 18 November 2016}\\      

==> TABLES/error_example.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll}
\toprule

Ambiguous Question& {Who was \textcolor{red}{\texttt{\textit{'the first act'}}} on live aid?} \\
Reference CQ from auto-conversion & {Could you clarify \textcolor{red}{\texttt{\textit{'the first act'}}}--\textcolor{blue}{\texttt{'at wembley stadium'}}, \textcolor{blue}{\texttt{'at john f. kennedy stadium'}}} \\
% , prior to the first musical act', or 'performance at john f. kennedy stadium , prior to the first musical act'?} \\
Generated CQ from BART & {Could you clarify \textcolor{red}{\texttt{\textit{'the first act'}}}--\textcolor{blue}{\texttt{'in the us'}} or \textcolor{blue}{\texttt{'in the uk'}}?}  \\\cline{1-2}

Ambiguous Question& {Who is \textcolor{red}{\texttt{\textit{'the speaker of the house'}}} in \textcolor{red}{\texttt{\textit{'california'}}}?} \\
Reference CQ from auto-conversion & {Could you clarify \textcolor{red}{\texttt{\textit{'california'}}}--\textcolor{blue}{\texttt{'2017'}}, \textcolor{blue}{\texttt{'2016'}}, or \textcolor{blue}{\texttt{'2014'}}?} \\
Generated CQ from BART & {Could you clarify \textcolor{red}{\texttt{\textit{'the speaker of the house'}}}--\textcolor{blue}{\texttt{'52nd'}} or   \textcolor{blue}{\texttt{'51st'}}?}  \\\cline{1-2}
% (`the speaker of the house', `52nd')-DQ& \texttt{Who is the speaker of the house \textbf{52nd} in california?} \\
% (`the speaker of the house', `51st')-DQ& \texttt{Who is the speaker of the house \textbf{51st} in california?} \\ \cline{1-2}

% Ambiguous Question& \texttt{Who sings in next to me imagine dragons?} \\
% Reference CQ from auto-conversion & \texttt{Could you clarify 'sings'--'lead vocals next to me by imagine dragons' or 'background vocals next to me by imagine dragons'?} \\
% Generated CQ from BART & \texttt{Could you clarify 'next to me imagine dragons'--'the lead vocals for' or 'the backing vocals for'?}  \\
% (`next to me imagine dragons', `the lead vocals for')-DQ& \texttt{Who sings in next to me by. imagine dragons \textbf{the lead vocals for} ?} \\
% (`next to me imagine dragons', `the backing vocals for')-DQ& \texttt{Who sings in next to me imaginge dragons \textbf{the backing vocals for}?} \\\cline{1-2}

% (`the first act', `in the us')-DQ& \texttt{Who has the first act \textbf{in the us} on live aid?} \\
% (`the first act', `in the uk')-DQ& \texttt{Who has the first act \textbf{in the uk} on live aid?} \\\cline{1-2}
Ambiguous Question& {\textcolor{red}{\texttt{\textit{'Who'}}} won \textcolor{red}{\texttt{\textit{'the men's figure skating 2018 olympics'}}}?} \\
Reference CQ from auto-conversion & {Could you clarify \textcolor{red}{\texttt{\textit{'Who'}}}--\textcolor{blue}{\texttt{'who was the individual'}} or \textcolor{blue}{\texttt{'what country'}}?} \\
Generated CQ from BART & {Could you clarify \textcolor{red}{\texttt{\textit{'the men's figure skating 2018 olympics'}}}--\textcolor{blue}{\texttt{'gold'}} or \textcolor{blue}{\texttt{'silver'}?}}  \\\cline{1-2}
% (`the men's figure skating 2018 olympics', `gold')-DQ& \texttt{Who won the men's figure skating 2018 olympics \textbf{gold}?} \\
% (`the men's figure skating 2018 olympics', `silver')-DQ& \texttt{Who won the men's figure skating 2018 olympics \textbf{silver}?} \\\cline{1-2}

Ambiguous Question& {Who \textcolor{red}{\texttt{\textit{'played'}}} mark on the tv show \textcolor{red}{\texttt{\textit{'roseanne'}}}?} \\
Reference CQ from auto-conversion & {Could you clarify \textcolor{red}{\texttt{\textit{'played'}}}--\textcolor{blue}{\texttt{'plays healy'}} or \textcolor{blue}{\texttt{'conner-healy'}}?} \\
Generated CQ from BART & {Could you clarify \textcolor{red}{\texttt{\textit{'roseanne'}}}--\textcolor{blue}{\texttt{'the original'}} or \textcolor{blue}{\texttt{'the revival'}}?}  \\\cline{1-2}
% (`roseanne', `the original')-DQ& \texttt{Who played mark on the tv show roseanne \textbf{the original}?} \\
% (`roseanne', `the revival')-DQ& \texttt{Who played mark on the tv show roseanne \textbf{the revival}?} \\\cline{1-2}

Ambiguous Question& {Who sings \textcolor{red}{\texttt{\textit{'youre the biggest part of me'}}}?} \\
Reference CQ from auto-conversion & {Could you clarify \textcolor{red}{\texttt{\textit{'the biggest part of me'}}}--\textcolor{blue}{\texttt{'what band'}} or \textcolor{blue}{\texttt{'lead vocal in'}}?} \\
Generated CQ from BART & {Could you clarify \textcolor{red}{\texttt{\textit{'youre the biggest part of me'}}}--\textcolor{blue}{\texttt{'in 1980'}} or \textcolor{blue}{\texttt{'in 2005'}}?}  \\
% (`youre the biggest part of me', `in 1980')-DQ& \texttt{Who sings youre the biggest part of me \textbf{in 1980}?} \\
% (`youre the biggest part of me', `in 2005')-DQ& \texttt{Who sings youre the biggest part of me \textbf{in 2005}?} \\
\bottomrule
\end{tabular}%
}
\caption{
Additional examples of clarification questions. We use the concatenation of the question, predicted answer, and relevant passage titles and contents as input.
}
\label{tab:error_ex}
\end{table*}


% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lll}
% \cline{1-1}
%                                   &  &  \\ \cline{1-1}


% \begin{tabular}[c]{@{}l@{}}AQ:   Who won the men's figure skating 2018 olympics?\\      Auto-converted: Could you clarify 'Who'--'who was the individual' or 'what country'??\\      Model-generated: Could you clarify 'the men's figure skating 2018 olympics'--'gold' or'silver'?\end{tabular} &  &  \\
% \multicolumn{1}{r}{Answers: Yuzuru Hanyu | Japan}                                                                                                                                                                                                               &  &  \\ \cline{1-1}

% \begin{tabular}[c]{@{}l@{}}AQ:   Who played mark on the tv show roseanne?\\      Auto-converted: Could you clarify 'played'--'plays healy' or 'conner-healy'?\\      Model-generated: Could you clarify 'roseanne'--'the original' or 'the revival'?\end{tabular} &  &  \\
% \multicolumn{1}{r}{Answers: Glenn Quinn | Ames McNamara}                                                                                                                                                                                                               &  &  \\ \cline{1-1}

% \begin{tabular}[c]{@{}l@{}}AQ:   Who sings youre the biggest part of me?\\      Auto-converted: Could you clarify 'the biggest part of me'--'what band' or 'lead vocal in'?\\      Model-generated: Could you clarify 'youre the biggest part of me'--'in 1980' or 'in 2005'?\end{tabular} &  &  \\
% \multicolumn{1}{r}{Answers: Ambrosia | David Robert Pack}                                                                                                                                                                                                               &  &  \\ \cline{1-1}
% \end{tabular}%
% }
% \caption{
% asdfasdfas
% }
% \label{tab:my-table}
% \end{table*}
% % option, ap 만 잡아도 됨. AP만 색깔로 하는걸 본문에 넣고 appendix 에 투컬럼으로 




% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{ll}
% \toprule

% Ambiguous Question& \texttt{Who was the first act on live aid?} \\
% Reference CQ from auto-conversion & \texttt{Could you clarify \textbf{'the first act'}--\textbf{'at wembley stadium'}, \textbf{'at john f. kennedy stadium'}} \\
% % , prior to the first musical act', or 'performance at john f. kennedy stadium , prior to the first musical act'?} \\
% Generated CQ from BART & \texttt{Could you clarify \textbf{'the first act'}--\textbf{'in the us'} or \textbf{'in the uk'}?}  \\\cline{1-2}

% Ambiguous Question& \texttt{Who is the speaker of the house in california?} \\
% Reference CQ from auto-conversion & \texttt{Could you clarify \textbf{'california'}--\textbf{'2017'}, \textbf{'2016'}, or \textbf{'2014'}?} \\
% Generated CQ from BART & \texttt{Could you clarify \textbf{'the speaker of the house'}--\textbf{'52nd'} or   \textbf{'51st'}?}  \\\cline{1-2}
% % (`the speaker of the house', `52nd')-DQ& \texttt{Who is the speaker of the house \textbf{52nd} in california?} \\
% % (`the speaker of the house', `51st')-DQ& \texttt{Who is the speaker of the house \textbf{51st} in california?} \\ \cline{1-2}

% % Ambiguous Question& \texttt{Who sings in next to me imagine dragons?} \\
% % Reference CQ from auto-conversion & \texttt{Could you clarify 'sings'--'lead vocals next to me by imagine dragons' or 'background vocals next to me by imagine dragons'?} \\
% % Generated CQ from BART & \texttt{Could you clarify 'next to me imagine dragons'--'the lead vocals for' or 'the backing vocals for'?}  \\
% % (`next to me imagine dragons', `the lead vocals for')-DQ& \texttt{Who sings in next to me by. imagine dragons \textbf{the lead vocals for} ?} \\
% % (`next to me imagine dragons', `the backing vocals for')-DQ& \texttt{Who sings in next to me imaginge dragons \textbf{the backing vocals for}?} \\\cline{1-2}

% % (`the first act', `in the us')-DQ& \texttt{Who has the first act \textbf{in the us} on live aid?} \\
% % (`the first act', `in the uk')-DQ& \texttt{Who has the first act \textbf{in the uk} on live aid?} \\\cline{1-2}
% Ambiguous Question& \texttt{Who won the men's figure skating 2018 olympics?} \\
% Reference CQ from auto-conversion & \texttt{Could you clarify \textbf{'Who'}--\textbf{'who was the individual'} or \textbf{'what country'}?} \\
% Generated CQ from BART & \texttt{Could you clarify \textbf{'the men's figure skating 2018 olympics'}--\textbf{'gold'} or \textbf{'silver'}?}  \\\cline{1-2}
% % (`the men's figure skating 2018 olympics', `gold')-DQ& \texttt{Who won the men's figure skating 2018 olympics \textbf{gold}?} \\
% % (`the men's figure skating 2018 olympics', `silver')-DQ& \texttt{Who won the men's figure skating 2018 olympics \textbf{silver}?} \\\cline{1-2}

% Ambiguous Question& \texttt{Who played mark on the tv show roseanne?} \\
% Reference CQ from auto-conversion & \texttt{Could you clarify \textbf{'played'}--\textbf{'plays healy'} or \textbf{'conner-healy'}?} \\
% Generated CQ from BART & \texttt{Could you clarify \textbf{'roseanne'}--\textbf{'the original'} or \textbf{'the revival'}?}  \\\cline{1-2}
% % (`roseanne', `the original')-DQ& \texttt{Who played mark on the tv show roseanne \textbf{the original}?} \\
% % (`roseanne', `the revival')-DQ& \texttt{Who played mark on the tv show roseanne \textbf{the revival}?} \\\cline{1-2}

% Ambiguous Question& \texttt{Who sings youre the biggest part of me?} \\
% Reference CQ from auto-conversion & \texttt{Could you clarify \textbf{'the biggest part of me'}--\textbf{'what band'} or \textbf{'lead vocal in'}?} \\
% Generated CQ from BART & \texttt{Could you clarify \textbf{'youre the biggest part of me'}--\textbf{'in 1980'} or \textbf{'in 2005'}?}  \\
% % (`youre the biggest part of me', `in 1980')-DQ& \texttt{Who sings youre the biggest part of me \textbf{in 1980}?} \\
% % (`youre the biggest part of me', `in 2005')-DQ& \texttt{Who sings youre the biggest part of me \textbf{in 2005}?} \\
% \bottomrule
% \end{tabular}%
% }
% \caption{
% Additional examples of clarification questions. We use the concatenation of the question, predicted answer, and relevant passage titles and contents as input.
% }
% \label{tab:error_ex}
% \end{table*}


% % \begin{table*}[t]
% % \centering
% % \resizebox{\textwidth}{!}{%
% % \begin{tabular}{lll}
% % \cline{1-1}
% %                                   &  &  \\ \cline{1-1}


% % \begin{tabular}[c]{@{}l@{}}AQ:   Who won the men's figure skating 2018 olympics?\\      Auto-converted: Could you clarify 'Who'--'who was the individual' or 'what country'??\\      Model-generated: Could you clarify 'the men's figure skating 2018 olympics'--'gold' or'silver'?\end{tabular} &  &  \\
% % \multicolumn{1}{r}{Answers: Yuzuru Hanyu | Japan}                                                                                                                                                                                                               &  &  \\ \cline{1-1}

% % \begin{tabular}[c]{@{}l@{}}AQ:   Who played mark on the tv show roseanne?\\      Auto-converted: Could you clarify 'played'--'plays healy' or 'conner-healy'?\\      Model-generated: Could you clarify 'roseanne'--'the original' or 'the revival'?\end{tabular} &  &  \\
% % \multicolumn{1}{r}{Answers: Glenn Quinn | Ames McNamara}                                                                                                                                                                                                               &  &  \\ \cline{1-1}

% % \begin{tabular}[c]{@{}l@{}}AQ:   Who sings youre the biggest part of me?\\      Auto-converted: Could you clarify 'the biggest part of me'--'what band' or 'lead vocal in'?\\      Model-generated: Could you clarify 'youre the biggest part of me'--'in 1980' or 'in 2005'?\end{tabular} &  &  \\
% % \multicolumn{1}{r}{Answers: Ambrosia | David Robert Pack}                                                                                                                                                                                                               &  &  \\ \cline{1-1}
% % \end{tabular}%
% % }
% % \caption{
% % asdfasdfas
% % }
% % \label{tab:my-table}
% % \end{table*}
% % % option, ap 만 잡아도 됨. AP만 색깔로 하는걸 본문에 넣고 appendix 에 투컬럼으로 



==> TABLES/input_example.tex <==
% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{ll}
% \toprule
% na-P& \texttt{who is the current chairman of african   union commission?\textless{}/s\textgreater{}\textless{}/s\textgreater \textbf{nkosazana dlamini-zuma}\textless{}/s\textgreater on 15...} \\
% pred-P & \texttt{who is the current chairman of african union commission?\textless{}/s\textgreater   \textless{}sep\textgreater  \underline{nkosazana   dlamini-zuma}\textless{}/s\textgreater \textbf{nkosazana dlamini-zuma}\textless{}/s\textgreater on 15...} \\
% gt-P & \texttt{who is the current chairman of african union commission?\textless{}/s\textgreater   \textless{}sep\textgreater  \underline{moussa faki}   \textless{}sep\textgreater  \underline{nkosazana dlamini-zuma}   \textless{}sep\textgreater  \underline{jean ping}\textless{}/s\textgreater   \textbf{nkosazana dlamini-zuma}\textless{}/s\textgreater on 15...}  \\ \cline{1-2}

% \bottomrule
% \end{tabular}%
% }
% \caption{
% Example of input to the CQ generation model. Each setting shows the prompt example listed in order of question, multiple answers (underlined), passage title(bold), passage content.  na-P refers to the input without multiple answers, pred-P refers to input with predicted answers from SPANSEQGEN and gt-P refers to input with ground truths from AMBIGNQ. As shown in the table, the number of predicted answers and the number of ground truth can be different.
% }
% \label{tab:cq_examples}
% \end{table*}


\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lll}
\cline{1-2}
                         & {\texttt{who is the current chairman of african   union commission?\textless{}/s\textgreater{}\textless{}/s\textgreater\textbf{nkosazana}}}\\                                                              & {\texttt{\textbf{dlamini-zuma}\textless{}/s\textgreater on 15 july 2012...\textless{}/s\textgreater\textbf{chairperson of the african union commission}}}           
                         
                         &  \\
\multirow{-3}{*}{none-P}   & {\texttt{</s>chairperson of the african...\textless{}/s\textgreater \textbf{erastus j.o.mwencha}\textless{}/s\textgreater erastus j.o.menwencha...}}                                                                                                             &  \\\cline{1-2}
                         & {\texttt{who is the current chairman of african   union commission?\textless{}/s\textgreater   \textless{}sep\textgreater  \underline{nkosazana   dlamini-zuma} }}     \\      
                         & {\texttt{\textless{}/s\textgreater \textbf{nkosazana dlamini-zuma}\textless{}/s\textgreater on 15 july 2012...\textbf{chairperson of the african union}}}     
                         
                         &  \\
                         
\multirow{-3}{*}{pred-P} & {\texttt{\textbf{commission}</s>chairperson of the african...\textless{}/s\textgreater \textbf{erastus j.o.mwencha}\textless{}/s\textgreater erastus...}}    &  
\\\cline{1-2}
                      
                         & {\texttt{who is the current chairman of african   union commission?\textless{}/s\textgreater   \textless{}sep\textgreater  \underline{moussa faki}\textless{}sep\textgreater  }} \\
                             & {\texttt{   \underline{nkosazana dlamini-zuma}\textless{}sep\textgreater  \underline{jean ping}\textless{}/s\textgreater\textbf{nkosazana dlamini-zuma}\textless{}/s\textgreater on 15 july 2012...}} &  \\
\multirow{-3}{*}{gt-P}   & {\texttt{\textbf{chairperson of the african union commission}......</s> chairperson of the...\textless{}/s\textgreater \textbf{erastus}...}}\\
\cline{1-2}
\end{tabular}%
}
\caption{
Input examples to the CQ generation model. Each example is a concatenation of question, multiple answers (underlined), and a sequence of relevant passages' titles (bold) and contents. 
}
\label{tab:input_ex}
\end{table*}






==> sec_results_and_discussion.tex <==
\section{Results and Discussion}
To solve our clarification question generation task, we fine-tuned BART$_\text{large}$ for 6 epochs.
Each of training prompt was a [SEP]-concatenation of an ambiguous question, its ground-truth multiple answers, and relevant passages.
As neural QA models for the extrinsic evaluation, we used a BART$_{\text{large}}$ fine-tuned on \textsc{NQ-OPEN} and its further fine-tuned one on human-annotated disambiguated questions and their answers provided in \textsc{AmbigNQ} for \hl{???} epochs.
As for the relevant passages, we used re-ranked ones across all experiments.  
We truncate all inputs up to 512 tokens due to our memory limitation.
Refer to Appendix~{??} for the detailed experimental setups.
% However, unlike the scheme, the model needs to predict clarification questions without annotated disambiguated questions.
